A machine learning approach for fighting the curse of dimensionality in global optimization

Finding global optima in high-dimensional optimization problems is extremely challenging since the number of function evaluations required to sufficiently explore the search space increases exponentially with its dimensionality. Furthermore, multimodal cost functions render local gradient-based search techniques ineffective. To overcome these difficulties, we propose to trim uninteresting regions of the search space where global optima are unlikely to be found by means of autoencoders, exploiting the lower intrinsic dimensionality of certain cost functions; optima are then searched over lower-dimensional latent spaces. The methodology is tested on benchmark functions and on multiple variations of a structural topology optimization problem, where we show that we can estimate this intrinsic lower dimensionality and based thereon obtain the global optimum at best or superior results compared to established optimization procedures at worst.

==> charcount.tex <==

!!! File not found or not readable: figures/tikz/Figure_13.tex !!!
(errors:1)
Word: Freq
All words: 0
---
Sum of subset: 0


==> wordcount.tex <==

!!! File not found or not readable: figures/tikz/Figure_13.tex !!!
(errors:1)

